KernelHaven -- An Open Infrastructure for Product Line Analysis

KernelHaven is an open infrastructure for Software Product Line (SPL) analysis. It is intended both as a production-quality analysis tool set as well as a research support tool, e.g., to support researchers in systematically exploring research hypothesis. For flexibility and ease of experimentation KernelHaven components are plug-ins for extracting certain information from SPL artifacts and processing this information, e.g., to check the correctness and consistency of variability information or to apply metrics. A configuration-based setup along with automatic documentation functionality allows different experiments and supports their easy reproduction. Here, we describe KernelHaven as a product line analysis research tool and highlight its basic approach as well as its fundamental capabilities. In particular, we describe available information extraction and processing plug-ins and how to combine them. On this basis, researchers and interested professional users can rapidly conduct a first set of experiments. Further, we describe the concepts for extending KernelHaven by new plug-ins, which reduces development effort when realizing new experiments.

==> SPLC18 - Demo - Arxiv/capabilities.tex <==
\section{Capabilities}
\label{sec:Capabilities}
The flexibility in combining and exchanging extractors and processing plug-ins is one of KernelHaven’s core capabilities, which, in particular, aims at supporting different users to conduct their desired analysis. As a starting point, different plug-ins are publicly available, which can be used out of the box. In this section, we introduce them by, first, discussing available extractors, their purpose, and extracted information and, second, describing realized processing plug-ins and their possible combinations with the extractors.\trim

KernelHaven provides seven different extractors as summarized in Table~\ref{tab:extractors}. Most of these extractors are \textbf{code extractors}. They rely on the code model illustrated in a simplified form in Figure~\ref{fig:Code Model} to provide code information of different granularity: ranging from code blocks to entire Abstract Syntax Trees (ASTs). This range of expressiveness is required to support a variety of external tools wrapped as KernelHaven plug-ins, like \textbf{Undertaker} \cite{Undertaker}, \textbf{srcML} \cite{srcML}, and \textbf{TypeChef} \cite{TypeChef}. Except for Undertaker, which is typically available as native Linux binary, these extractors are executable on any operating system. Due to this limitation of Undertaker, we also provide a reimplementation of its algorithms in Java resulting in the operating-system-independent and faster \textbf{Code Block} extractor. Hence, both extractors extract conditional code blocks (right side of Figure~\ref{fig:Code Model}) from C-code files defined as input in Table~\ref{tab:extractors}. In contrast, srcML and TypeChef provide ASTs of their input files, which results in a set of possibly nested \texttt{SyntaxElement}s as illustrated on the left side of Figure~\ref{fig:Code Model}. While the AST of the srcML extractor currently only provides a granularity of single line statements\footnote{This is due to the ongoing work on this extractor; the original srcML tool provides more details.}, the TypeChef extractor enables variability-aware parsing including macro-expansion\footnote{TypeChef automatically considers header files (\texttt{*.h}) without an explicit definition of those files as input.}, which results in significantly more details about code files.\trim
%KernelHaven provides seven different extractors as summarized in Table~\ref{tab:extractors}. Most of these extractors are \textbf{code extractors}, which wrap external tools, like \textbf{Undertaker} \cite{Undertaker}, \textbf{srcML} \cite{srcML}, and \textbf{TypeChef} \cite{TypeChef}. Except for Undertaker, which is typically available as native Linux binary, these extractors are executable on any operating system. Due to this limitation of Undertaker, we also provide a reimplementation of its algorithms in Java resulting in the operating-system-independent and faster \textbf{Code Block} extractor. Hence, both extractors extract conditional code blocks from C-code files defined as input in Table~\ref{tab:extractors}. In contrast, srcML and TypeChef  provide Abstract Syntax Trees (ASTs) of their input files. While the AST of the srcML extractor currently only provides a granularity of single line statements\footnote{This is due to the ongoing work on this extractor; the original srcML tool provides more details.}, the TypeChef extractor enables variability-aware parsing including macro-expansion\footnote{TypeChef automatically considers header files (\texttt{*.h}) without an explicit definition of those files as input.}, which results in a fine-grained AST.

% ################### EXTRACTORS TABLE ###################
\begin{table}
	\caption{Available KernelHaven extractors (April 2018)}
	\begin{threeparttable}
	\centering
		\begin{tabulary}{\columnwidth}{LLLLL}
			\hline
			\textbf{Name} & \textbf{Type} & \textbf{Input} & \textbf{OS} \\ \hline \hline
			Undertaker\tnote{1} & Code & *.c/*.h/*.S & Linux \\ \hline
			Code Block\tnote{2} & Code & *.c/*.h/*.S & Any \\ \hline
			srcML\tnote{1} & Code & *.c/*.h & Any \\ \hline
			TypeChef\tnote{1} & Code & *.c & Any \\ \hline
			KBuildMiner\tnote{1} & Build & KBuild/Make & Any \\ \hline
			KConfigReader\tnote{1} & VM & Kconfig & Linux \\ \hline
			DIMACSVariabilityModel\tnote{2} & VM & DIMACS & Any \\ \hline
		\end{tabulary}
		\begin{tablenotes}
			\footnotesize
			\item VM = Variability Model 
			\item[1] This extractor wraps an external tool not developed by the authors
			\item[2] This extractor is solely developed by the authors
		\end{tablenotes}
	\end{threeparttable}
	\label{tab:extractors}
\end{table}
% ################### EXTRACTORS TABLE ###################

The \textbf{KBuildMiner} extractor is the only publicly available \textbf{build extractor} so far. It wraps the corresponding tool \cite{KBuildMiner}, which takes KBuild- and Make-files as input and provides the mapping of files and presence conditions as described in Section~\ref{sec:Overview}. In particular, KBuild-files stem from the Linux kernel build system \cite{Kbuild18} and its specific variability realization technique, which uses \texttt{CONFIG\_*} symbols in code and build files to reference configuration options defined in the variability model. Hence, this extractor explicitly searches for such references to build the mapping. Build extractors for other variability realization techniques can easily be implemented by exploiting the extensibility features described in Section~\ref{sec:Extensibility}.\trim

The \textbf{KConfigReader} and the \textbf{DIMACSVariabilityModel} extractors represent two fundamentally different \textbf{variability model extractors}. While the former wraps the KConfigReader tool \cite{KConfigReader}, which explicitly takes Kconfig-files \cite{Kbuild18} as input and uses build tools of the Linux kernel restricting its applicability to Linux only, the latter extracts propositional formulas in DIMACS format and converts them into the internal variability model representation of KernelHaven on any operating system. Similar to the KBuildMiner build extractor, KConfigReader is the extractor of choice if an experiment requires variability model information from the Linux kernel build system. The DIMACSVariabilityModel extractor can be used, for example, for any SPL using a feature model as this type of model can be easily translated into propositional formulas \cite{Batory05} and, hence, into DIMACS format.

KernelHaven allows any combination of the above extractors for a specific experiment. However, the actual processes and algorithms implemented in a processing plug-in may require a particular setup of the pipelines. Table~\ref{tab:processings} includes such dependencies for the available processing plug-ins as an example. The \textbf{UnDeadAnalysis} detects dead code blocks or missing features as described in \cite{TartlerLohmannSincero+11}. Therefore, it requires the respective block information from code files, which multiple code extractors provide. Hence, one of them needs to be defined in the respective KernelHaven configuration file. Further, the analysis requires build information to determine whether the code file including the respective code block is part of the final product. The availability of a particular file and its inherent code blocks is typically controlled by configuration options defined in the variability model, which requires a corresponding extractor.%\trim

% ################### PROCESSING TABLE ###################
\begin{table*}[!bt]
	\caption{Available KernelHaven processing plug-ins and possible extractor combinations (July 2018)}
	\vspace*{-1em}
	\begin{threeparttable}
	\centering
		\begin{tabular}{lp{5cm}p{3cm}ll}
			\hline
			\textbf{Name} & \textbf{Goal} & \textbf{Code Extractor} & \textbf{Build Extractor} & \textbf{VM Extractor} \\ \hline \hline
			% previously used \tnote{1} to reference table note items below
			UnDeadAnalysis\textsuperscript{1} & Detection of dead code blocks (never part of any product) or missing features & Undertaker, Code Block, srcML, or TypeChef & KBuildMiner & KConfigReader \\ \hline
			ConfigurationMismatches\textsuperscript{2} & Detection of inconsistencies between modeled and effective variability & \multicolumn{3}{p{8cm}}{\centering\textit{Processes the results of the FeatureEffect analysis and, hence, \newline does not directly use a particular extractor}} \\ \hline
			FeatureEffect\textsuperscript{1} & Reverse engineering of variability constraints from code and build files to improve an existing or create a new VM & Undertaker, Code Block, srcML, or TypeChef & KBuildMiner & \textit{not required}\\ \hline
			MetricHaven\textsuperscript{1,2} & More than 7,300 metrics and their variants for measuring SPL properties & srcML (TypeChef possible, but not realized yet) & KBuildMiner & KConfigReader \\ \hline
		\end{tabular}
		\begin{tablenotes}
			\footnotesize
			% Squeeze multiple items in one line; requires manual references in terms of \textsuperscript{1}
			\item VM = Variability Model; \textsuperscript{1} This processing is a reimplementation in KernelHaven of existing work; \textsuperscript{2} This processing is developed by the authors
			%\item VM = Variability Model
			%\item[1] This processing is a reimplementation in KernelHaven of existing work
			%\item[2] This processing is solely developed by the authors
		\end{tablenotes}
	\end{threeparttable}
	\label{tab:processings}
	\vspace*{-7pt}
\end{table*}
% ################### PROCESSING TABLE ###################

The \textbf{FeatureEffect} analysis requires a different setup of KernelHaven as it is a reverse engineering approach, which identifies variability constraints from code and build files \cite{NadiBergerKastner+15}. Hence, it does not need a variability model extractor as well as the respective pipeline. For this purpose, a user simply excludes the corresponding parameters from KernelHaven’s configuration file. Further, the \textbf{ConfigurationMismatches} analysis builds upon the same configuration as it uses the results of the feature effect analysis to check whether the implemented (effective) variability matches the variability model \cite{El-SharkawyKrafczykSchmid17}. This concatenation of processing plug-ins results in processing or analysis pipelines, which we describe in detail in \cite{KroeherEl-SharkawySchmid18}. In essence, processing pipelines are defined by combining processing plug-ins in the order they consume their results in the configuration file without any further implementation effort.

A fundamentally different type of experiment is represented by \textbf{MetricHaven}. This processing plug-in
%consists of a set of variability-aware implementation metrics and their variants
provides currently more than 7,300 metric variations \cite{El-SharkawyYamagishi-EichlerSchmid17} to measure SPL artifact types in isolation as well as in combination. Similar to the \textbf{UnDeadAnalysis}, this plug-in requires all pipelines and, in particular, srcML as it provides the necessary implementation details.

The set of already available plug-ins shows the potential of KernelHaven to support various types of experiments ranging from verification and analyses to metrics. A user can conduct these experiments with different levels of details, e.g., code blocks or entire ASTs, depending on the configured extractors. Further, new plug-ins can be realized and combined with the existing ones to extend the current capabilities as described in the following section.


==> SPLC18 - Demo - Arxiv/conclusion.tex <==
\vspace*{-1ex}
\section{Conclusion}
\label{sec:Conclusion}
We presented KernelHaven as an experimentation workbench to support different types of users in their goal to conduct their individual experiments in the domain of static Software Product Line (SPL) analyses and verification.  Users benefit from the available plug-ins, which wrap some of the most prominent analysis tools in this domain and, hence, simplify their application even in new experiments. KernelHaven addresses researchers by explicitly supporting the documentation and reproduction of experiments. Developers take advantage of the rather simple extensibility due to reusability of existing plug-ins and abstraction from technical details provided by the core infrastructure.
We believe that KernelHaven is also applicable in teaching SPL engineering as it significantly reduces time and effort students need to setup a particular extraction, analysis, metric, etc. Rather, it is simply a matter of extracting an archive and executing KernelHaven with the desired configuration.


==> SPLC18 - Demo - Arxiv/extensibility.tex <==
\section{Extensibility}
\label{sec:Extensibility}
\begin{figure}[t]
	\centering
    %trim={<left> <lower> <right> <upper>,clip}
		\includegraphics[trim={3.5cm 9.35cm 6.3cm 2.8cm},clip,width=\columnwidth]{figures/CodeModel.pdf}
  %\vspace{-4ex}
	\caption{Simplified code model of KernelHaven}
	\label{fig:Code Model}
	%\vspace{-1em}
\end{figure}
The architecture of KernelHaven is designed to simplify the development of new extensions by means of separation of concerns and reuse. This allows researchers to focus on the realization of novel concepts while abstracting from technical details. We outline the three design concepts for achieving this simplicity in this section.

\textbf{Decoupled extractors and processing.} Independent data models decouple the extraction of relevant information and the processing of the extracted data. On the one side, this facilitates the reuse of already developed processing plug-ins for new artifact types as only a new extractor is required. One the other side, the realization of novel processing algorithms, e.g., a new code metric, may reuse existing extractors for already handled artifact types.

\textbf{Reuse of processing algorithms.} KernelHaven processing plug-ins do not differentiate between the output of extractors or other processing plug-ins. Thus, new processing plug-ins may reuse existing and mature processing plug-ins to form a processing or analysis pipeline, like the concatenation of the feature effect and configuration mismatches analyses in Section~\ref{sec:Capabilities}. In this way, developers can realize complex processing algorithms incrementally. Individual KernelHaven plug-ins may represent these increments, which can be used both in isolation as well as in combination with other processing algorithms and, hence, avoid extra effort for re-implementing required processing capabilities. 

\textbf{Abstraction from technical details.} The KernelHaven infrastructure separates conceptual work from technical implementation. This way, researchers do not need to consider aspects like multithreading or saving of results as the infrastructure takes care of that. This means that KernelHaven executes by default all extraction pipelines (cf.\ Figure~\ref{fig:Architecture}) and all processing plug-ins in parallel. For instance, the configuration mismatch analysis may start to validate that the variability model covers the detected code dependencies of the feature effect analysis, while this analysis still detects further code dependencies. However, developers can force all processing components (extractors or processing plug-ins) to complete before a new component starts. To save the results, a developer only needs to annotate data classes and KernelHaven takes care of storing the results. Thus, developers usually neither need to specify any output formats nor to take care of stream handling.


==> SPLC18 - Demo - Arxiv/intro.tex <==
\section{Introduction}
\label{sec:Introduction}
KernelHaven is a tool for supporting professional research, in particular, in the area of Software Product Line (SPL) analysis and verification. In order to provide optimal research support, it rests on the underlying metaphor of an \textit{experimentation workbench}: it is explicitly designed to support rapid evaluation of various research hypotheses, easy creation of different setups in the exploration stage, reuse of research results, and support of reproducibility and documentation as described in \cite{KroeherEl-SharkawySchmid18}. It thus aims to support researchers in conducting experiments in a similarly broad way as a development workbench like Eclipse supports a developer.

While KernelHaven explicitly focuses on product line analysis and verification, it aims to support a wide range of tasks in this domain and due to its openness is closer to an open ecosystem than to a product line. As we discuss in Section~\ref{sec:Overview}, it currently supports (up to) three different input pipelines, which are fed into a processing step typically addressing analysis or verification activities. 
All individual steps in extraction and processing can be realized by different, independent plug-ins, creating a broad range of possible applications. There exist already a significant number of publicly available plug-ins. Some are actually  wrapped components of well-known research tools like Undertaker~\cite{Undertaker} or TypeChef~\cite{TypeChef}, while others have been developed as part of the KernelHaven-project\footnote{\label{fn:Website}\url{https://github.com/KernelHaven}}. Due to the integration framework that KernelHaven offers, it is easy to set up an experiment combining code analysis from Undertaker with a variability analysis using KConfigReader~\cite{KConfigReader}. And it is also a matter of minutes to determine whether results differ, if as an alternative for code-analysis the Code Block extraction plug-in is used.
As a practical consideration it is sometimes also important that as a result of this clear separation into plug-ins, the various tools may have different licenses and can still be used in combination as long as the user is allowed to use each individual part.\trim
 
In its current form, especially given the currently available plug-ins, KernelHaven is well equipped for Linux-related analysis. However, we emphasize, that there is no architectural restriction in this regard. Rather, it can be used for any type of product line and any type of static analysis. The architecture is indeed so open that it can also be used itself as some form of post- or pre-processing in other scientific analysis. We are currently investigating such applications. 

Besides the support for research, the well-defined packaging of the various plug-ins allows to apply these analyses more easily and flexibly in industry. We experienced this in some of our industrial cooperations, where the framework greatly enhanced the usability also for the industrial partners \cite{El-SharkawyJyotiKrafczyk+18}.  

The remainder of this paper is structured as follows: Section~\ref{sec:Overview} provides a short overview of the basic architecture of the tool. Section~\ref{sec:Capabilities} then looks more in-depth into the current capabilities, in particular, the different available plug-ins. The intention is to provide a better understanding of the out-of-the-box capabilities of the tool as it is available right now. 
Section~\ref{sec:Extensibility} reviews the  approach for extensibility of the framework. This is particularly relevant to anyone aiming to integrate fundamentally new analysis approaches. Finally, in Section~\ref{sec:Conclusion}, we conclude.


==> SPLC18 - Demo - Arxiv/meta/acknowledgment.tex <==
\vspace*{-1ex}
\begin{acks}
This work is partially supported by the ITEA3 project $\text{REVaMP}^2$, funded by the \grantsponsor{01IS16042H}{BMBF (German Ministry of Research and Education)}{https://www.bmbf.de/} under grant \grantnum{01IS16042H}{01IS16042H}. Any opinions expressed herein are solely by the authors and not by the BMBF.
  
We thank the following contributors: Moritz Fl\"oter, Adam Krafczyk, Alice Schwarz, Kevin Stahr, Johannes Ude, Manuel Nedde, Malek Boukhari, and Marvin Forstreuter.
\end{acks}


==> SPLC18 - Demo - Arxiv/meta/docSettings.tex <==
\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{setspace}
\usepackage[flushleft]{threeparttable} % for creating tables with table notes
\usepackage{tabulary} % for creating tables with pre-defined width and automatic text wrapping
\usepackage{dblfloatfix}
\usepackage{framed} % for printing gray box illustrating the execution command (see 'Command' below)
\usepackage{xcolor} % for printing gray box illustrating the execution command (see 'Command' below)

% Table settings
\usepackage{csvsimple}

%\include{meta/showMargins}

% For include graphics
\usepackage{graphicx}

\usepackage{hyperref} 
\hypersetup{
    pdfauthor={Christian Kröher, Sascha El-Sharkawy, and Klaus Schmid},
    pdftitle={KernelHaven - An Open Infrastructure for Supporting Software Product Line Engineering},
    pdfsubject={22st International Conference on Software Product Line},
    pdfkeywords={Software product lines; variability modeling; reverse engineering; static analysis},
    pdfpagemode={UseOutlines},
    pdfproducer={LaTeX},
    colorlinks=true,
    linkcolor=black,          % color of internal links
    citecolor=black,          % color of links to bibliography
    filecolor=black,          % color of file links
    urlcolor=black            % color of external links
}


% Spacing
% Less space before and after floating elements (figures, listings, tables, ...)
\setlength{\textfloatsep}{4pt plus 1.0pt minus 2pt}
\renewcommand{\bottomfraction}{.5}

% Custom configuration of enumerations (lists)
\usepackage{enumitem}
\setlist[itemize]{leftmargin=1em}
\setlist[enumerate]{leftmargin=3ex}
\setlist[description]{leftmargin=1em}


% Hurenkinder und Schusterjungen verhindern
\clubpenalty10000
\widowpenalty10000
\displaywidowpenalty=10000
% Weniger Woerter trennen
\sloppy

% Balancing last page
%\usepackage{flushend}

% Command Box
\colorlet{shadecolor}{gray!25}
\newcommand{\Command}[1]{
  %\begin{minipage}[t]{0.925\columnwidth}
    \begin{snugshade*}
      \noindent #1
    \end{snugshade*}
  %\end{minipage}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                     %%%
%%% Self-defined Macros %%%
%%%                     %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\trim}{\looseness-1}
\newcommand{\ifDef}{\texttt{\#ifdef}}


==> SPLC18 - Demo - Arxiv/meta/lstSettings.tex <==
\definecolor{cEclipseRed}{rgb}{0.6,0,0}
\definecolor{cEclipseGreen}{rgb}{0.25,0.5,0.35}
\definecolor{cEclipsePurple}{rgb}{0.5,0,0.35}
\definecolor{cEclipseBlue}{rgb}{0.25,0.35,0.75}

% Listings
%\usepackage{textcomp}              % straight quotes
\usepackage{listings}
\lstset{
  backgroundcolor=\color{white},                   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  basicstyle=\ttfamily\small,                      % the size of the fonts that are used for the code
  breakatwhitespace=false,                         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                                 % sets automatic line breaking
  breakindent=10pt,
	captionpos=b,                                    % sets the caption-position to bottom
  %columns=fullflexible,                            % en-/dis-able same space for all characters (cf. https://tex.stackexchange.com/a/300132)
	commentstyle=\color{cEclipseGreen},              % comment style
  deletekeywords={...},                            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},                          % if you want to add LaTeX within your code
  extendedchars=true,                              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  frame=single,                                    % adds a frame around the code
  framesep=1pt,
  keepspaces=true,                                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\bfseries\color{cEclipsePurple},    % keyword style
  %language=Octave,                                % the language of the code
  morekeywords={*,...},                            % if you want to add more keywords to the set
  numbers=left,                                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                                   % how far the line-numbers are from the code
  numberstyle=\tiny\color{gray!70!black},          % the style that is used for the line-numbers
  postbreak=\mbox{\textcolor{red}{$\hookrightarrow$}},
	rulecolor=\color{black},                         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,                          % underline spaces within strings only
  showtabs=false,                                  % show tabs within strings adding particular underscores
  stepnumber=1,                                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{cEclipseBlue},                % string literal style
  tabsize=4,                                       % sets default tabsize to 2 spaces
  %title=\lstname                                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  xleftmargin=1.25em,
  %upquote=true,
  linewidth=.98\columnwidth
}

% Java
\lstdefinelanguage{j} {
    language=Java,
    keywordstyle=[2]{\color{gray!70!black}},
    morekeywords=[2]{@Override},
}

% Properties
\lstdefinelanguage{properties} {
    tabsize=1,
    commentstyle=\color{blue}, 
    morecomment=[s][\color{cEclipsePurple}]{<}{>},
		morecomment=[l]{\	},
    morecomment=[l][\color{cEclipseGreen}]{\#},		
}


==> SPLC18 - Demo - Arxiv/meta/meta_acm.tex <==
% #### Title and Authors ####
\title{KernelHaven---An Open Infrastructure for Product Line Analysis}
\author{Christian Kröher, Sascha El-Sharkawy, Klaus Schmid}
\affiliation{
  \institution{University of Hildesheim, Institute of Computer Science}
  \streetaddress{Universit{\"a}tsplatz 1}
  \city{Hildesheim}
	\country{Germany}
  \postcode{31134}
}
\email{{kroeher, elscha, schmid}@sse.uni-hildesheim.de}
% #### Title and Authors ####


% #### Abstract ####
\begin{abstract}
KernelHaven is an open infrastructure for Software Product Line (SPL) analysis. It is intended both as a production-quality analysis tool set as well as a research support tool, e.g., to support researchers in systematically exploring research hypothesis. For flexibility and ease of experimentation KernelHaven components are plug-ins for extracting certain information from SPL artifacts and processing this information, e.g., to check the correctness and consistency of variability information or to apply metrics. A configuration-based setup along with  automatic documentation functionality allows different experiments and supports their easy reproduction.

Here, we describe KernelHaven as a product line analysis research tool and highlight its basic approach as well as its fundamental capabilities. In particular, we describe available information extraction and processing plug-ins and how to combine them. 
On this basis, researchers and interested professional users can rapidly conduct a first set of experiments. Further, we describe the concepts for extending KernelHaven by new plug-ins, which reduces development effort when realizing new experiments.
\end{abstract}
% #### Abstract ####


% #### Concepts and Keywords ####
%
% The code below should be generated by the tool at
% http://dl.acm.org/ccs.cfm
% Please copy and paste the code instead of the example below. 
%
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10002944.10011123.10010912</concept_id>
<concept_desc>General and reference~Empirical studies</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10002944.10011123.10011131</concept_id>
<concept_desc>General and reference~Experimentation</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10011007.10011074.10011092.10011096.10011097</concept_id>
<concept_desc>Software and its engineering~Software product lines</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}
\ccsdesc[500]{General and reference~Empirical studies}
\ccsdesc[500]{General and reference~Experimentation}
\ccsdesc[500]{Software and its engineering~Software product lines}
\keywords{Software product line analysis, variability extraction, static analysis, empirical software engineering}
% #### Concepts and Keywords ####


% ### Copyright ###
\copyrightyear{2018}
\acmYear{2018}
\setcopyright{rightsretained}
\acmConference[SPLC '18]{22nd International Systems and Software
Product Line Conference - Volume B}{September 10--14,
2018}{Gothenburg, Sweden}
\acmBooktitle{22nd International Systems and Software Product Line
Conference - Volume B (SPLC '18), September 10--14, 2018, Gothenburg,
Sweden}\acmDOI{10.1145/3236405.3236410}
\acmISBN{978-1-4503-5945-0/18/09}
% ### Copyright ###


\maketitle


==> SPLC18 - Demo - Arxiv/meta/showMargins.tex <==
% See: https://tex.stackexchange.com/a/271294
\usepackage{showframe}
\usepackage{etoolbox}
\newlength\Fcolumnseprule
\setlength\Fcolumnseprule{0.4pt}

\makeatletter
\newcommand\ShowInterColumnFrame{
\patchcmd{\@outputdblcol}
  {{\normalcolor\vrule \@width\columnseprule}}
  {\vrule \@width\Fcolumnseprule\hfil
    {\normalcolor\vrule \@width\columnseprule}
    \hfil\vrule \@width\Fcolumnseprule
  }
  {}
  {}
}

\makeatother
\ShowInterColumnFrame

==> SPLC18 - Demo - Arxiv/meta/todos.tex <==
\ifshowToDos
  % Force margin par, even if not allowed by acm
  \usepackage{marginnote} 
  \setlength{\marginparwidth}{1.5cm}
  \let\marginpar\marginnote
  
  % ToDos
  \newcommand{\ToDo}[1]{\noindent\fcolorbox{black}{yellow!20!white}{\parbox{.975\columnwidth}{#1}}}
  \newcommand{\SubjectedToDo}[2]{\ToDo{\textbf{#1:}#2}}
  \newcommand{\ToDoInline}[1]{\fcolorbox{black}{yellow!20!white}{#1}}
  \newcommand{\Outline}[1]{\color{blue}{#1}\color{black}}
  \newcommand{\Problem}[1]{\color{red}{#1}\color{black}}
  \newcommand{\secSize}[1]{[#1]}
  
  % Comments
  \usepackage[textsize=small,colorinlistoftodos]{todonotes}
  % Comment as ToDo note per author. First argument is color, second is the text
  \newcommand{\userComment}[2]{\todo[color=#1!20,linecolor=#1!60,bordercolor=#1!60]{#2}}
  \newcommand{\ks}[1]{\userComment{orange}{\textbf{KS:} #1}}
  \newcommand{\se}[1]{\userComment{red}{\textbf{SE:} #1}}
  \newcommand{\ak}[1]{\userComment{blue}{\textbf{AK:} #1}}
  \newcommand{\ck}[1]{\userComment{green}{\textbf{CK:} #1}}
  \newcommand{\sjd}[1]{\userComment{yellow}{\textbf{SYD:} #1}}
  
  % Checkmark for ToDos and comments
  \usepackage{pifont}
  \newcommand{\cmark}{\ding{51}}
\else
  % Disable ToDos
  \newcommand{\ToDo}[1]{}
  \newcommand{\SubjectedToDo}[2]{}
  \newcommand{\ToDoInline}[1]{#1} % Verwende ich für Zahlen, die sich noch ändern können
  \newcommand{\Outline}[1]{}
  \newcommand{\Problem}[1]{}
  \newcommand{\secSize}[1]{}
  
  % Disable comments
  \newcommand{\ks}[1]{}
  \newcommand{\se}[1]{}
  \newcommand{\ak}[1]{}
  \newcommand{\sd}[1]{}
	\newcommand{\ck}[1]{}
\fi

==> SPLC18 - Demo - Arxiv/overview.tex <==
\section{Overview}
\label{sec:Overview}
KernelHaven is designed to support a variety of similar experiments in the domain of static SPL analysis and verification \cite{KroeherEl-SharkawySchmid18}. This design enables rapid prototyping as well as detailed analyses by offering an open plug-in infrastructure implemented in Java. The core components of this infrastructure are three extraction pipelines, the data processing, and a pipeline configurator as illustrated in Figure~\ref{fig:Architecture} and described in this section.

Each \textbf{pipeline} extracts and provides information of a particular type of artifact typically considered in variability-based analyses:

\begin{itemize}
	\item The code pipeline in the upper part of Figure~\ref{fig:Architecture} extracts information from code files resulting in a set of element trees. An element tree represents a single code file and provides information about the available code elements on different levels of abstraction. We provide more details on this data model in Section~\ref{sec:Capabilities}.
\item The build pipeline in the middle of Figure~\ref{fig:Architecture} extracts and provides information from build files. The result of this extraction is a map of files and their presence conditions (PC in Figure~\ref{fig:Architecture}) \cite{DietrichTartlerSchroderPreikschat+12, NadiHolt12}. These conditions define constraints, which must be satisfied to compile and link or, in general, build a specific (set of) file(s).
\item The (variability) model pipeline in the lower part of Figure~\ref{fig:Architecture} translates information from variability model files into a list of features and propositional formulas. They represent the features and constraints, which define the planned products of the SPL.
\end{itemize}

The quality of the extracted information depends on the specific extractors defined for the individual pipelines. Extractors can be easily exchanged by adapting the configuration file described later in this section. This exchangeability allows, e.g., to use a fast but imprecise extractor for early experiments, which serve the improvement of the experiments core processes and algorithms, and to switch to a rather slow but detailed extractor for final results.

The information provided by one or multiple pipelines is input to the core \textbf{processes and algorithms} of the conducted experiment. As experiments can be of different nature, the particular processing of the input information depends on the desired results. Hence, this processing can be exchanged similar to the extractors. We discuss the already available processing variants in Section~\ref{sec:Capabilities}, ranging from static analysis and verification tasks to software metrics. A particular feature of KernelHaven processing plug-ins is that they can call other processing plug-ins to consume their results, like the configuration mismatch analysis described in Section~\ref{sec:Capabilities}. Hence, there can be a complete sub-pipeline for processing, too.

The \textbf{configuration} file in the lower left part of Figure~\ref{fig:Architecture} defines the particular setup of an experiment and, hence, a specific instance of KernelHaven. It consists of a set of parameters for preparing the infrastructure (input and output locations, etc.) as well as defining the required pipelines, the desired extractors, and processing plug-ins. The pipeline configurator reads these parameters to configure KernelHaven prior to its execution.

Besides these core components and the resulting flexibility in setting up different experiments, KernelHaven also offers features, which particularly address common research challenges \cite{Boettiger15, CitoGall16, EichelbergerSassSchmid16}: comprehensive documentation and reproduction of experiments. KernelHaven supports automatic archiving of all relevant plug-ins, input, output, and intermediate data along with its core infrastructure. Further, the resulting archive contains the configuration file, which defines the experimental setup and, hence enables reproduction of an entire experiment on a new machine. This only requires the installation of Java on an operating system, which the extractors of the experiment support. In the following section, we explicitly include these dependencies on specific operating systems as part of our discussion of existing KernelHaven capabilities.

\begin{figure}[t] % t für top, b = bottom, h = here
	\centering
		%trim={<left> <lower> <right> <upper>}
		\includegraphics[width=\columnwidth,trim={6,8cm 7,1cm 6,5cm 5,1cm},clip]{figures/KernelHaven-Architecture.pdf}
  \caption{KernelHaven architecture}
	\label{fig:Architecture}
\end{figure}


==> meta/showMargins.tex <==
% See: https://tex.stackexchange.com/a/271294
\usepackage{showframe}
\usepackage{etoolbox}
\newlength\Fcolumnseprule
\setlength\Fcolumnseprule{0.4pt}

\makeatletter
\newcommand\ShowInterColumnFrame{
\patchcmd{\@outputdblcol}
  {{\normalcolor\vrule \@width\columnseprule}}
  {\vrule \@width\Fcolumnseprule\hfil
    {\normalcolor\vrule \@width\columnseprule}
    \hfil\vrule \@width\Fcolumnseprule
  }
  {}
  {}
}

\makeatother
\ShowInterColumnFrame
